Probabilistic Automata of Bounded Ambiguity

Probabilistic automata are an extension of nondeterministic finite automata in which transitions are annotated with probabilities. Despite its simplicity, this model is very expressive and many of the associated algorithmic questions are undecidable. In this work we focus on the emptiness problem (and its variant the value problem), which asks whether a given probabilistic automaton accepts some word with probability greater than a given threshold. We consider a natural and well-studied structural restriction on automata, namely the degree of ambiguity, which is defined as the maximum number of accepting runs over all words. The known undecidability proofs exploits infinite ambiguity and so we focus on the case of finitely ambiguous probabilistic automata. Our main contributions are to construct efficient algorithms for analysing finitely ambiguous probabilistic automata through a reduction to a multi-objective optimisation problem called the stochastic path problem. We obtain a polynomial time algorithm for approximating the value of probabilistic automata of fixed ambiguity and a quasi-polynomial time algorithm for the emptiness problem for 2-ambiguous probabilistic automata. We complement these positive results by an inapproximability result stating that the value of finitely ambiguous probabilistic automata cannot be approximated unless PTIME = NP.

==> review <==

First review:

# Review on the paper
# Probabilistic Automata of Bounded Ambiguity
# by N. Fijalkow, C. Riveros, J. Worrell
# submitted to Information and Computation
# special issue on "Weighted automata"

* Summary
Probabilistic automata (PA) form a well-studied extension of finite
automata with probabilistic transitions. Unfortunately, most
interesting decision problems are undecidable for this class of
models. In this submission, the authors study how bounding the
ambiguity of probabilistic automata can make decision problems
decidable.

More precisely, they focus on two central problems: the *emptiness
problem* (input: a PA, and a threshold; output: yes iff there exists a
word accepted with probability greater than the threshold), and the
*value problem* (input: a PA; output: the supremum over finite words
of acceptance probability). For PA, the emptiness problem is
undecidable, and the value is neither computable nor approximatable.

An observation is that the undecidability proof for the emptiness
problem of unrestricted PA uses automata with an unbounded ambiguity
degree. The /ambiguity degree/ of an automaton (here, probabilities do
not matter) is a function from naturals to naturals which assigns to a
natural n the maximum over all words w of length n of the number of
accepting runs over w. It is thus natural to study whether bounding
the ambiguity makes the emptiness problem decidable, and the
computation of the value feasible.

A very recent result from the litterature (which appeared after the
conference paper this journal submission is based on) is that the
emptiness problem remains undecidable for /linearly ambiguous/ PA,
that is, PA for which the ambiguity degree is bounded by a
first-degree polynomial. The authors thus naturally consider /finitely
ambiguous/ PA. Note that one can refine the class of finitely
ambiguous PA into
- P-ambiguous PA: ambiguity degree is bounded by P(|Q|), where Q is
   the state space of the input PA
- k-ambiguous PA: ambiguity degree is bounded by constant k

The contributions of this submission are the following
- The emptiness problem is
   - PSPACE-hard an in NEXPTIME for finitely ambiguous PA;
   - PSPACE-complete for P-ambiguous PA;
   - in NP for k-ambiguous PA; and
   - in quasipolynomialTIME for 2-ambiguous PA.
- The value problem is
   - not approximable (in polynomial time within a constant factor)
     unless P=NP; and
   - approximable in polynomial time within any constant c>1 for
     k-ambiguous PA.

* Evaluation - Detailed comments

The idea of restricting the ambiguity of PA to hope for decidability
results is quite natural. Yet, the contributions of this paper seem
novel. As far as I could judge, the results are sound. The
contributions are not groundbreaking in my opinion. Most proof
techniques are not new, to the exception of the ones involving the
multi-stochastic path problem. Compared to the conference version, I
would be happy to see more useful details. For instance, I would
expect fully detailed proofs (rather than reduction on an example). I
would also expect the paper to be self-contained, and not use notions
(directed ideals, PosSLP, etc) that are --in my opinion-- non
standard. The added value compared to the conference version is
somehow limited... On the positive side, it fits the topic of the
special issue "Weighted automata". The authors should be advised to
carefully proof-read their article before submission.

- Some proofs are not detailed, and the authors only give
   intuitions. This might be fine for the conference version, but I
   would expect full details in a journal version. In particular, for a
   reduction proof, I expect to be given the reduction. This applies
   typically to the proof of Theorem 3, for which the construction is
   only given on an example. I finally understood the reduction, yet I
   think it should be given in the general case. Moreover, some fact is
   wrong in that proof (see below).
*****
The proof of Theorem 3 is now given in full details. 
*****

- I might be worth mentioning that for k-ambiguous automata, the value
   is a maximum (the supremum is reached). I think it is related to
   Lemma 1.

*****
We added it in the statement of Lemma 1.
*****

- The PosSLP problem is not even defined. Beyond a reference, I would
   expect a definition of this decision problem.

*****
We took a different approach: since the PosSLP problem is only used once in one a (non-central) complexity bound, and defining it properly would take a lot of space,
we reformulated this item. Suffices to say that there exists a PSPACE algorithm for checking whether an arithmetic circuit has value greater than a given threshold (which indeed is called the PosSLP problem).
*****

- You use the term k-stochastic path problem. Why not use 2-stochastic
   path problem when k=2? Alternatively, keep bi-stochastic, and then
   use multi-stochastic.

*****
Agreed, thanks!
*****

- I would use (1+ \varepsilon)-approximation, rather than
   \varepsilon-approximation. I think this is the correct
   terminology. For instance the traveller salesman problem admits a
   2-approximation --rather than a 1-approximation-- when the
   "distance" function is Eulerian.

*****
Agreed, thanks!
*****

- Add "References" before the references.

*****
Agreed, thanks!
*****

* Minor comments
** General comments
- Please use \emph{} consistently for i.e., e.g., and so on: that is
   either never or always.

*****
Agreed, thanks!
*****

- Please choose betwen \epsilon and \varepsilon.

*****
Agreed, thanks!
*****

** Abstract
- You write you "focus on the emptiness problem". I suggest to add
   "and the value problem".

*****
Agreed, thanks!
*****

- "We observe that undecidability of the emptiness problem requires
   infinite ambiguity". Rather, the known undecidability proof exploits
   infinite ambiguity. Am I wrong?

*****
Agreed, thanks!
*****

** Introduction
- The first time "bounded ambiguity" is mentionned, the notion has not
   been defined.

*****
The definition comes in the next sentence.
*****

- Please add a reference to Chadha et al 2018 and Daviaud et al 2018
   in the 4th paragraph of the introduction.

*****
Agreed, thanks!
*****

- page 3, line 5: automaton -> automata

*****
Agreed, thanks!
*****

** Section 2
- I find it unappropriate to use the same notation ($\mathcal{P}$) for
   three purposes: a PA, its induced probability measure, and the
   acceptance probability of a word!

*****
We understand your concern, but this does not introduce any ambiguity, and it saves space for indices (another notation would be Prob_\P, which uses the index), we kept it as it is.
*****

- Page 5: a polynomial ambiguous automaton -> a polynomially ambiguous
   automaton

*****
Agreed, thanks!
*****

- Page 5: About the classification in PTIME of the ambiguity degree
   (Weber and Seidl), I would suggest removing "probabilistic", since
   (1) the result was not proved in that context, and (2) anyway this
   notion only depends on the underlying non-probabilistic automaton.

*****
Agreed, thanks!
*****

** Section 3
- Page 5: which justifies -> which justify

*****
Agreed, thanks!
*****

- Page 6: of the Post Correspondence's Problem -> of Post's
   Correspondence Problem [3 errors]

*****
Agreed, thanks!
*****

- Page 7: does there exist -> whether there exists

*****
Agreed, thanks!
*****

- Page 7: to continuous \Sigma^\omega maps on -> to continuous maps on
   \Sigma^\omega

*****
Agreed, thanks!
*****

- Page 7: < 2^n should read < 2^{-n}

*****
Agreed, thanks!
*****

- Page 7: "the linearly ambiguous PA" What PA do you refer to here? I
   guess it is obtained from the one of Figure 1, but it should depend
   on the PCP instance one starts with... Please give more details in
   that proof.

*****
We expanded that proof.
*****

- Proof of Th2: the last three lines are not rigorously formulated (or
   at least the way they are written is ambiguous). I would write that
   for fixed \varepsilon and w, |bin(\varphi_1(w)) - bin(\varphi_2(w))|
   \leq \varepsilon iff |\mathcal{P}(w) - 1/2| \leq \varepsilon. Hence
   the following equivalence: (\forall \varepsilon \exists w |bin -
   bin| \leq \varepsilon) iff (\forall \varepsilon \exists w |P(w) -
   .5| \leq \varepsilon).

*****
Reformulated.
*****

- "We proved undecidability results". Some of these were established
   by others. Please reformulate.


*****
Agreed, thanks!
*****

** Section 4
- Please add a reference end of Page 8, about the inapproximability of
   the maximum clique problem.

*****
Reformulated.
*****

- "In P_G a word over {a,b}^* represents a set of vertices". I think
   you rather want to write that "a word in {a,b}^n represents a set of
   vertices".

*****
Reformulated.
*****

*** Proof of Theorem 3
- This proof has to be rewritten carefully.

*****
Entirely rewritten and expanded.
*****

- "the run corresponding to a vertex v is successful iff v and all its
   neighbours belong to the set of vertices represented by the word
   w". This statement seems wrong. On the illustrating example,
   consider w= aabb; the run on w corresponding to v_1 is accepted; v_3
   is a neighbour of v_1; however v_3 does not belong to the set
   encoded by w=aabb, the latter being {v_1,v_2}.

*****
Indeed, reformulated.
*****

- In the same proof, it is said that P_G has n runs on each
   word. However, the illustrating example has e.g. a single run on the
   word aaaa. I assume you want P_G to be complete, but this is not
   mentioned.

*****
There are n runs, but less accepting runs. We made this clearer.
*****

- "the size of the largest clique" -> "the size of a largest clique"

*****
Agreed, thanks!
*****

- I could not understand how the factor 2^{n-1} is dealt with at the
   end of the proof. Also, what is K? An arbitrary function that bounds
   the approximation factor?

*****
Further explained.
*****

** Section 5
- and threshold c -> and a threshold c

*****
Agreed, thanks!
*****

- Unfortunately the proof of regularity -> Unfortunately our proof of
   regularity

*****
Agreed, thanks!
*****

- The notions of ideal, downward closed and directed sets are not
   defined (even informally).

*****
Agreed, thanks!
*****

- "\mathbb{N}^k is a well quasi order" Please rephrase: \mathbb{N}^k
   must be equipped with the natural order.

*****
Agreed, thanks!
*****

- subset of D \subseteq \mathbb{N}^k -> subset D of \mathbb{N}^k

*****
Agreed, thanks!
*****

- \Delta(p,q)(q) -> \Delta(p,a)(q)

*****
Agreed, thanks!
*****

- there exists some k [] and some m -> there exist some k [...] and
   some m

*****
Agreed, thanks!
*****

- each set is downwards closed -> each set is downward closed

*****
Agreed, thanks!
*****

- a finitely ambiguous automata -> a finitely ambiguous automaton

*****
Agreed, thanks!
*****

- Page 12: in item 3, please replace u (resp. v) with x (resp. y) to
   be consistent with the above.

*****
Agreed, thanks!
*****

- This reduce -> This reduces

*****
Agreed, thanks!
*****

- p \leq q' -> p' \leq q

*****
Agreed, thanks!
*****

- (see Lemma 1) -> (see the proof of Lemma 1)

*****
Agreed, thanks!
*****

- in hand -> at hand

*****
We think it is correct to write "with these bounds in hand".
*****

- For k-ambiguous -> For k-ambiguous automata

*****
Agreed, thanks!
*****

- for finitely ambiguous -> for finitely ambiguous PA

*****
Agreed, thanks!
*****

- Page 13: correspond to decide PosSLP -> corresponds to deciding
   PosSLP

*****
Sentence reformulated.
*****

** Section 6
- progress on the literature of -> progress in the literature on

*****
Agreed, thanks!
*****

- can have different edges -> can have several edges

*****
Agreed, thanks!
*****

- "weights are computed multiplicatively" Please rephrase: weights are
   fixed; the way they are aggregated into a quantity is by
   multiplication.

*****
Agreed, thanks!
*****

- The statement of Lemma 2 is not rigorous enough. Please rephrase the
   sentence not to mix instances and decision problems.

*****
Agreed, thanks!
*****

- which of two k runs are different -> which pairs of runs are different?

*****
Agreed, thanks!
*****

- accordingly to -> according to

*****
Agreed, thanks!
*****

- "the previous explanation" What do you have in mind here?

*****
Reformulated.
*****

- You might want to use \mathbb{0} for example for the zero
   matrix. Otherwise, one does not see the difference with the
   length 0.

*****
Agreed, thanks!
*****

- is closely related to -> reduces in polynomial time to

*****
Agreed, thanks!
*****

- "Hence the introduction of two relaxation". This sentence is
   grammatically incorrect: it should contain a verb.

*****
Agreed, thanks!
*****

- showing which -> showing what

*****
Agreed, thanks!
*****

- The statement of Theorem 7 should be rewritten: "there exists a
   polynomial time algorithms [...] in time polynomial [...]".

*****
Agreed, thanks!
*****

- In the proof of Theorem 7, I find it weird to use the term bits
   although the encoding is in unary.

*****
Agreed, thanks!
*****

- I find it useless to redefine the value of a PA on page 18.

*****
Removed.
*****

- output Output -> return Output

*****
Agreed, thanks!
*****

- we start by showing -> we start by giving

*****
Agreed, thanks!
*****

- bi-objective shortest path problem -> bi-stochastic shortest path
   problem


*****
Agreed, thanks!
*****



*********************************************************************************

Second review:

Context:
=======

The paper studies finite probabilistic automata (PFA). A PFA is like a
nondeterministic finite automaton, but has probabilities associated to
transitions.
For each state and letter, the outgoing transitions determine a probability
distribution over the set of states. In this way, every word determines a
probability distribution over the set of states, too. Thus, a PFA
associates, with
every word, an acceptance probability (the probability of reaching a
final state).
PFA go back to Rabin and have been widely studied.

A fundamental decision problem asks whether there is a word whose acceptance
probability is greater  than a given threshold. It is well known that
this problem
is undecidable (Paz 1971; Bertoni 1974). It has recently been shown that
undecidability even holds for linearly ambiguous PFA, where the number
of accepting
runs grows only linearly with the length of a word.

Results:
=======

Here, the authors show that, under that restriction, the isolation
problem (do all
words have an acceptance probability that is not too close to a given
threshold?) is
already undecidable, too. To do so, they adapt a reduction by Bertoni,
which relies
on a variant of the PCP problem. In the following, the paper focuses on
k-ambiguous
PFA, for a fixed k, in which every word has at most k accepting runs.
Letting k
range over all natural numbers, one obtains the class of finitely
ambiguous PFA.
However, the authors first show a negative result: there is no
polynomial-time
approximation algorithm that approximates the value (the supremum of all
acceptance
probabilities) of finitely ambiguous PFA (unless P=NP). The proof is by
reduction
from the maximum clique size problem for which it has been known that it
is hard to
approximate.

On the positive side, the authors first show that the threshold language
of every
finitely ambiguous PFA is regular, which is in general not the case
(Rabin 1963),
unless the threshold is isolated. The proof is via a nice argument using
ideal
decompositions of downward-closed subsets of \mathbb{N}^k. Towards an
efficient
emptiness test (which is not guaranteed by the previous result), the
authors then
go on to show that only words up to length n^k (n being the number of
states) need
to be considered. In fact, when k is not explicitly given, words of length
exponential in n are sufficient. Using these insights, it is shown that:
* Emptiness checking for k-unambiguous PFA (for fixed k) is in NP.
* Emptiness checking for PFA with p-bounded ambiguity (for fixed
polynomial p) is
   in PSPACE.
* Emptiness checking for finitely ambiguous PFA is in NEXPTIME.

The paper concludes with an interesting polynomial-time reduction of the
emptiness
problem for k-ambiguous PFA to the k-stochastic path problem. This
finally leads to
a polynomial-time approximation algorithm as well as a quasi-polynomial-time
algorithm for checking emptiness of 2-ambiguous PFA.

Evaluation and Conclusion:
=====================

This is a nice paper, which sheds light on a couple of intriguing
decision problems
around natural subclasses of probabilistic automata. The paper is very
well written.
The presentation follows a logical structure so that each result appears
to be well
motivated. There is not much to complain about so that I recommend to
accept the
paper almost as is.

Minor comments:
==============

* page 6, line 11: Strictly speaking, the threshold language was defined
only for
   strict inequality.

*****
Reformulated
*****

* page 10, line 1: Please recall what k is.

*****
Done.
*****

* page 11, line -12 automata => automaton

*****
Thanks!
*****

* page 13, lines 5-6: strict vs non-strict inequality

*****
Changed.
*****

* page 14, line 2 of Section 6: emptines => emptiness

*****
Thanks!
*****

* page 14, line -6: I think you could explain “consecutive” formally.

*****
Reformulated.
*****

* page 15, Fig. 3 : The node labels s,p,q,t could be a bit larger.

*****
Agreed, thanks!
*****

* page 17, line -10: Please rephrase "showing which is sometimes ...".

*****
Agreed, thanks!
*****

* page 19, line -9: \epsilon => \varepsilon (to be consistent)

*****
Agreed, thanks!
*****

* page 20: A conclusion would be nice. Are there further interesting
directions
   for future work?

*****
We added a conclusion.
*****



